Preference Diffusion for Recommendation

Recommender systems predict personalized item rankings based on user preference distributions derived from historical behavior data. Recently, diffusion models (DMs) have gained attention in recommendation for their ability to model complex distributions, yet current DM-based recommenders often rely on traditional objectives like mean squared error (MSE) or recommendation objectives, which are not optimized for personalized ranking tasks or fail to fully leverage DM's generative potential. To address this, we propose PreferDiff, a tailored optimization objective for DM-based recommenders. PreferDiff transforms BPR into a log-likelihood ranking objective and integrates multiple negative samples to better capture user preferences. Specifically, we employ variational inference to handle the intractability through minimizing the variational upper bound and replaces MSE with cosine error to improve alignment with recommendation tasks. Finally, we balance learning generation and preference to enhance the training stability of DMs. PreferDiff offers three key benefits: it is the first personalized ranking loss designed specifically for DM-based recommenders and it improves ranking and faster convergence by addressing hard negatives. We also prove that it is theoretically connected to Direct Preference Optimization which indicates that it has the potential to align user preferences in DM-based recommenders via generative modeling. Extensive experiments across three benchmarks validate its superior recommendation performance and commendable general sequential recommendation capabilities. Our codes are available at https://github.com/lswhim/PreferDiff.

==> chapters/5_related_work.tex <==
\section{Related Work}
\textbf{Sequential Recommendation} have gained significant attention in both academia~\citep{recsysbook, SelfGNN} and industry~\citep{SeqRecSys, SeqRec} due to their ability to capture user preferences from historical interactions and recommend the next item. One common research line has focused on developing more efficient network architectures, such as GRU~\citep{GRU4Rec}, convolutional neural networks~\citep{CASER}, Transformer~\citep{SASRec, LightSAN}, Bert4Rec~\citep{Bert}, and HSTU~\citep{HSTU}. Another research line focuses on leveraging additional unsupervised signals~\citep{CL4Rec, ContraRec, RLMRec} or reshaping sequential recommendation into other tasks such as retrieval~\citep{TIGER, EAGER} and language generation~\citep{TallRec, E4SRec, LLaRa}.

\textbf{DM-based Recommenders} have been explored in recent studies due to the powerful generative and generalization capabilities of diffusion models (DMs)~\citep{DMRecSurvey}. These recommenders either focus on modeling the distribution of the next item (e.g., ~\citep{DreamRec, CDDRec, DiffuRec}), capture the probability distribution of user interactions (e.g., ~\citep{DiffRec, DDRM}), or focus on the distribution of time intervals between user behaviors (e.g., ~\citep{PDRec}). However, existing approaches often rely on conventional objectives, such as mean squared error (MSE), or standard recommendation-specific objectives like Bayesian Personalized Ranking (BPR)~\citep{BPR} and Cross Entropy (CE)~\citep{Goldloss}. We argue that the former may diverge from the core objective of accurately modeling user preference distributions in recommendation tasks~\citep{recsysbook}, as DMs often lack an adequate understanding of negative items. While the latter leverages DMs' noise resistance to mitigate noisy interactions in recommendations which might fall short of fully exploiting the generative and generalization capabilities of DMs.





